An Intermittent Click Planning Model

Pointing is the task of tracking a target with a pointer and confirming the target selection through a click action when the pointer is positioned within the target. Little is known about the mechanism by which users plan and execute the click action in the middle of the target tracking process. The Intermittent Click Planning model proposed in this study describes the process by which users plan and execute optimal click actions, from which the model predicts the pointing error rates. In two studies in which users pointed to a stationary target and a moving target, the model proved to accurately predict the pointing error rates (R2 = 0.992 and 0.985, respectively). The model has also successfully identified differences in cognitive characteristics among first-person shooter game players.

==> study3.tex <==

\section{Third Study}
The program which stores mouse and keyboard logs for this study is written in c++.
This program uses the interception library\cite{Lopes2015interception} and the Windows Driver Development Kit (WinDDK) to collect input values from the keyboard and mouse.
It stores event time, mouse movement distance and click event information in csv format whenever keyboard and mouse events occur.
The Gdiplus library is used to capture the screen. When the mouse is clicked, the screen is automatically captured and it is used to check the accuracy of the aim.
Since the screen capture function creates a heavy load on the main process, it is designed to work on a thread.

